Direct Telemetry Access

Fine-grained network telemetry is becoming a modern datacenter standard and is the basis of essential applications such as congestion control, load balancing, and advanced troubleshooting. As network size increases and telemetry gets more fine-grained, there is a tremendous growth in the amount of data needed to be reported from switches to collectors to enable network-wide view. As a consequence, it is progressively hard to scale data collection systems. We introduce Direct Telemetry Access (DTA), a solution optimized for aggregating and moving hundreds of millions of reports per second from switches into queryable data structures in collectors' memory. DTA is lightweight and it is able to greatly reduce overheads at collectors. DTA is built on top of RDMA, and we propose novel and expressive reporting primitives to allow easy integration with existing state-of-the-art telemetry mechanisms such as INT or Marple. We show that DTA significantly improves telemetry collection rates. For example, when used with INT, it can collect and aggregate over 400M reports per second with a single server, improving over the Atomic MultiLog by up to $16$x.

==> Sections/Motivation_old.tex <==
%\documentclass[../main.tex]{subfiles}
\graphicspath{{\subfix{../}}}
\begin{document}
    \begin{table}[]
        \centering
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{@{}lc@{}}
            \toprule
            \textbf{System} & \textbf{Per-switch Report Rate} \\ \midrule
            \textbf{INT Postcards} (Per-hop latency, 0.5\% sampling) & 19 Mpps\\
            \textbf{Marple~\cite{narayana2017language}} (TCP out-of-sequence) & 6.72 Mpps\\
            \textbf{Marple~\cite{narayana2017language}} (Packet counters) & 4.29 Mpps\\
            \textbf{NetSeer~\cite{zhou2020flow}} (Flow events) & 950 Kpps\\\bottomrule
        \end{tabular}
        }
        %\vspace*{1mm}
        \caption{Per-reporter data generation rates by various monitoring systems, as presented in their individual papers.\protect\footnotemark{}
        Numbers are based on 6.4Tbps switches.}
        \label{tab:motivation_system_speeds}
    %\vspace*{-0.15in}
    \end{table}
     \addtocounter{footnote}{-1}

    \begin{figure}[t]
        \centering
        \includegraphics[width=\columnwidth]{Figures/motiv_collection_costs_2.pdf}
        \caption{Number of required collection cores for various data center sizes, using telemetry systems proposed by the research community. \jl{Discuss, and explain num switches and hyperscale}}
        \label{fig:motiv_network_collection_cores}
    \end{figure}
    
    %\vspace*{-1mm}
    \section{Motivation}
    \label{sec:motivation}
    As telemetry systems move to fine-grained, real-time analysis and support network-wide queries, data collection becomes the key bottleneck. In this section, we quantify this bottleneck in existing systems, propose to use RDMA as the basic transport mechanism between switches and collectors, and discuss key challenges in adopting it.
    
    \vspace*{-2mm}
    \subsection{Collection overhead of telemetry systems}\label{sec:motivation_collection_costs}
    \jl{I think we are losing reviewers here. Our arguments why we need better performance (and RDMA) is not clear enough}
    \vbox{We investigated a few state-of-the-art telemetry systems and summarize the reporting rate generated by \emph{a single switch} in Table~\ref{tab:motivation_system_speeds}, based on the numbers in the corresponding papers\footnotemark.}
    \footnotetext{INT does not advertise a specific telemetry reporting rate, and we chose an arbitrary sampling rate of $0.5\%$ to keep overheads low, as an example.}
%    \minlan{We need to introduce different modes of INT here and analyze their overhead respectively, so sec 3 and table 2 can refer to them here}
    When using INT in postcard mode~\cite{intelINT} on a commodity 6.4Tbps switch, and considering a standard load of  ${\approx}$40\%~\cite{microburstfb}, it could generate up to $19M$ reports per second. 
    Other solutions are less demanding on collectors, either because pre-processing and filtering of data at switches reduces the reporting rate~\cite{zhou2020flow,gupta2018sonata}, or because they focus on more specific tasks that limit the data to report~\cite{narayana2017language}. For example, NetSeer~\cite{zhou2020flow} discusses a system that \mbox{exports just $950K$ records per second per switch.}
 
   
    To get a network-wide view, we may need to collect data from hundreds of thousands of switches in data center networks~\cite{guo2015pingmesh}. This means a network can easily generate billions of reports per second, even using a lightweight system such as NetSeer. For each report from a switch, collectors spend CPU cycles in I/O receiving the data. Even though DPDK greatly reduces the cost of packet I/O, polling traffic at $148$Mpps requires as much as $12$ dedicated CPU cores~\cite{dpdkNVIDIAPerf}. As a consequence, \emph{thousands of CPU cores} have to be dedicated \mbox{to \emph{just receive} billions of reports per second~\cite{langlet2021zero}.}
    
           \begin{figure}
    \vspace*{-5mm}
        \centering
        \includegraphics[width=1.0\linewidth]{Figures/motivation_confluo_breakdown_v12.pdf}    
        %\vspace*{-0.31mm}
        \caption{CPU-based collectors are inefficient. Shown above is the collection work breakdown of Confluo, the state-of-the-art collector for high-speed networks.}
        \label{fig:motivation_cpu_collector_breakdown}
        \vspace{-0.05in}
    \end{figure}
    
    Once the data is received, it has to be processed in the user-space to store the information in a queryable data structure. The processing usually involves three key operations that require more CPU cores: \emph{parsing} (extract content from the incoming report packets), \emph{data wrangling} (process the data to make it suitable for insertion, e.g., hashing it into a fixed-size key), and \emph{storing} (determine where to store it in memory). 
    
    While I/O is costly, this additional processing can be even more expensive. 
    Figure~\ref{fig:motivation_cpu_collector_breakdown} shows the breakdown of Confluo~\cite{khandelwal2019confluo}, the state-of-the-art collector for high-speed networks, when receiving and processing $100K$ reports on an Intel Xeon Silver 4114 CPU @ 2.20GHz. 
    Data wrangling in Confluo organizes the reports based on user criteria (e.g., filtering on event type). Storing involves batching, computing a key (indexing), and inserting reports into memory.  
    % insertion, where reports are scheduled to be written in memory.
    We found that most CPU cycles ($86\%$) are spent in data wrangling and storing, almost $11$x the cost of its I/O. 
    It is clear that optimizing the collector stacks is critical for minimizing {the number of cores used for \emph{data collection}~\cite{khandelwal2019confluo}.} \sivaram{May be this was removed, I think we had a graph to show this: Is it worth mentioning that we can potentially scale many servers to solve this problem?}\ga{We removed because we were not confident on Confluo costs. Do you have an idea on how to present them?}
   
    %\vspace*{-2mm}
    \subsection{Challenges for using RDMA}
    Our goal is to reduce the CPU utilization of collectors to scale with large numbers of telemetry reports from many switches. RDMA is a natural solution that has been already used to boost the performance of consensus protocols~\cite{sift}, reads in key-value stores~\cite{xstore,onesided-kvs}, and data replication~\cite{tailwind}.
    A strawman solution could have switches write their reports directly in collectors' memory with RDMA calls without CPU involvement. Although this idea appears attractive, and generating RDMA instructions directly from switches is possible~\cite{kim2020tea}, it presents challenges when applied to telemetry collection:
    
    \boldskipper
    \noindent\textbf{(1) RDMA verbs are limited.} Telemetry data has to be stored in the collectors' memory in such a way that it is then easy to query. For example, using data structures such as linked lists or cuckoo hash tables can reduce data retrieval times significantly~\cite{khandelwal2019confluo}. However, RDMA provides support for a limited set of operations: \emph{Read}, \emph{Write}, \emph{Fetch-and-Add}, and \emph{Compare-and-Swap}. This makes it hard to implement the data structures mentioned above, as they require us to first read memory at the collector before knowing exactly what to write and where, leading to significantly more complex on-switch logic and increased RDMA traffic. Enabling advanced RDMA offloads on commodity NICs is possible, but at the cost of a reduction of performance that can reach  2 orders of magnitude~\cite{reda2021rdma}. Furthermore, it not possible to support multiple RDMA senders writing at the same memory location while guaranteeing no conflicts or race conditions. This is paramount for network telemetry, where multiple {switches have to report their data to a collector. }
    
    \boldskipper
    %\vbox
    {
    \noindent\textbf{(2) A limited number of RDMA connections.} RDMA NICs can only handle a limited number of active connections (also known as \emph{queue pairs}) at high speed. %, due to limited on-NIC memory for RDMA statefulness. 
    Increasing the number of queue pairs degrades RDMA performance by up to 5x~\cite{dragojevic2014farm}. 
    This limits the total number of switches that can generate telemetry RDMA packets to a collector before performance starts degrading. 
    Alternatively, several switches can share the same queue pair, but RDMA imposes the assumption that every packet received at the collector has a strictly sequential ID, which is impractical for a distributed network of switches.
    }

    \iffalse
        \boldskipper
        \jl{Remove challenge 3}
        \noindent\textbf{(3) High-speed RDMA needs a lossless network.} An RDMA receiver expects incoming packets to be in sequential order. With packet loss, this expectation fails, leading to queue-pair invalidation which degrades RDMA performance~\cite{mittal2018revisiting}. For this reason, current deployments adopt per-hop flow-control mechanisms such as PFC~\cite{pfc} to rate-limit RDMA traffic in case of congestion~\cite{rdma-msr-15,timely,mittal2018revisiting}. Unfortunately, this can introduce deadlocks, a circular buffer dependency between switches that causes network throughput collapse~\cite{tagger}. 
        Worse, many switches reporting telemetry data at a collector increase the chances of incast, thus pushing PFC to kick in. As telemetry traffic would run on the data plane, it would force {applications' traffic to be subjected to PFC rules as well. }
    \fi
    
    \boldskipper
    \noindent\textbf{(3) Managing RDMA connections is costly for switches.} Programmable switches are not designed to generate RDMA telemetry packets. The standard protocol used for RDMA communication (RoCEv2) requires maintaining state for connections that can be expensive to implement. For instance, the switch has to store metadata,
    and generate appropriate headers and associated checksums. However, current programmable switches are limited in memory, computational \mbox{logic, and internal bus bandwidth.} 
\end{document}
